Fast and Uncertainty-Aware Directional Message Passing for Non-Equilibrium Molecules

Many important tasks in chemistry revolve around molecules during reactions. This requires predictions far from the equilibrium, while most recent work in machine learning for molecules has been focused on equilibrium or near-equilibrium states. In this paper we aim to extend this scope in three ways. First, we propose the DimeNet++ model, which is 8x faster and 10% more accurate than the original DimeNet on the QM9 benchmark of equilibrium molecules. Second, we validate DimeNet++ on highly reactive molecules by developing the challenging COLL dataset, which contains distorted configurations of small molecules during collisions. Finally, we investigate ensembling and mean-variance estimation for uncertainty quantification with the goal of accelerating the exploration of the vast space of non-equilibrium structures. Our DimeNet++ implementation as well as the COLL dataset are available online.

==> tables/dimenet_pp_embedding_sizes.tex <==
\begin{tabular}{ccccc}
	\toprule
	{int\_emb\_size} & {global\_emb\_size} & {out\_emb\_size} & {Time per epoch (minutes)} & {logMAE in eV}
	\midrule
	128 & 128 & 128 & 4.88 & -4.923229 \\
	32 & 128 & 128 & 3.51 & -4.837962 \\
	64 & 128 & 128 & 4.29 & -4.865119 \\
	64 & 64 & 128 & 3.08 & -4.618874 \\
	64 & 128 & 256 & 4.17 & -4.910487 \\
	64 & 128 & 512 & 4.31 & -5.012184 \\
\end{tabular}

==> tables/dimenet_pp_improvements_old.tex <==
\begin{tabular}{lccc}
	\toprule
	{Model (\& change made)} & {Layers} & {Time per epoch (minutes)} & {logMAE in eV} \\
	\midrule
	DimeNet & 6 & 34.38 & -4.794949 \\
	+ Hadamard product & 6  & 6.37 & -4.661383 \\
	+ Hadamard + MLP for RBF, SBF & 6 & ? & ? \\
	\midrule
	${\mathrm{DimeNet}}^h$ (num\_blocks: 8) & 8   & 11.00 & -4.806845 \\
	${\mathrm{DimeNet}}^h$ (num\_blocks: 4) $\to\ {\mathrm{DimeNet}}^{hb}$ & 4  & 5.84 & \textbf{-4.812865} \\
	${\mathrm{DimeNet}}^h$ (num\_blocks: 3) & 3  &  4.13 & -4.790296 \\
	\midrule
	\midrule
	${\mathrm{DimeNet}}^{hb}$ (int\_emb\_size: -) & 4 & 5.84 & -4.812865 \\
	${\mathrm{DimeNet}}^{hb}$ (int\_emb\_size: 32) & 4  & 3.94 & -4.809433 \\
	${\mathrm{DimeNet}}^{hb}$ (int\_emb\_size: 64) & 4  & 4.65 & \textbf{-4.861783} \\
	\midrule
	${\mathrm{DimeNet}}^{hb}$ (2-layer MLP for SBF)  & 4  & 5.84 & -4.812865 \\
	${\mathrm{DimeNet}}^{hb}$ (no MLP for SBF)  & 4  & 4.81 & -4.718217 \\
	${\mathrm{DimeNet}}^{hb}$ (2-layer MLP for both RBF and SBF) & 4  & 6.28 & \textbf{-4.863081} \\
	\midrule
	${\mathrm{DimeNet}}^{hb}$ (global\_emb\_size: 128, out\_emb\_size:128) & 4  & 5.84 & -4.812865 \\
	${\mathrm{DimeNet}}^{hb}$ (global\_emb\_size: 64, out\_emb\_size:128) & 4  & 3.78 & -4.634749 \\
	${\mathrm{DimeNet}}^{hb}$ (global\_emb\_size: 128, out\_emb\_size:256) & 4  & 4.34 & \textbf{-4.890271} \\
	\toprule
\end{tabular}


==> tables/uq.tex <==
\begin{tabular}{l@{\hspace{0.2cm}}c@{\hspace{0.2cm}}c@{\hspace{0.2cm}}c@{\hspace{0.2cm}}c@{\hspace{0.2cm}}c@{\hspace{0.2cm}}c@{\hspace{0.2cm}}}
	 & Time per epoch & RMSE$_E$ & RMSE$_\mF$ & {$\rho(\Delta_E,\sigma_E)$} & {$\rho(\Delta_\mF,\sigma_\mF)$} & {$\rho(\Delta_\mF,\sigma_E)$}\\
	\hline
	SchNet & \textbf{\SI{5.4}{\minute}} & 0.372 & 0.400 & - & - & -\\
	DimeNet$^{++}$ & \SI{9.3}{\minute} & ? & ? & - & - & -\\
	Ensemble & \SI{28.0}{\minute} & \textbf{0.188} & \textbf{0.266} &  0.34  &  0.80 & 0.33\\
	MVE & \SI{7.4}{\minute} & 0.251 & 0.272 & 0.34 & - & 0.17\\
\end{tabular}
% Time per 1k steps converted via (9_000 / 32 + 1_000 / 32 / 2) / (1_000 + 1_000 / 32 / 2) = 0.2923076923076923
% Time per 10k steps converted via (9_000 / 32 + 1_000 / 32 / 2) / (10_000 + 1_000 / 32 / 2) = 0.029641185647425898
% Scale to 70k+10k: (70_000 + 10_000 / 2) / (9_000 + 1_000 / 2)
